An Unsupervised Probability Model for Speech-to-Translation Alignment of Low-Resource Languages

For many low-resource languages, spoken language resources are more likely to be annotated with translations than with transcriptions. Translated speech data is potentially valuable for documenting endangered languages or for training speech translation systems. A first step towards making use of such data would be to automatically align spoken words with their translations. We present a model that combines Dyer et al.'s reparameterization of IBM Model 2 (fast-align) and k-means clustering using Dynamic Time Warping as a distance metric. The two components are trained jointly using expectation-maximization. In an extremely low-resource scenario, our model performs significantly better than both a neural model and a strong baseline.

==> examples/speaker-example.tex <==
\begin{tikzpicture}[scale=0.4]

\pgfmathsetmacro{\SPA}{18}
\pgfmathsetmacro{\MA}{16}
\pgfmathsetmacro{\SPB}{10}
\pgfmathsetmacro{\MB}{8}
\pgfmathsetmacro{\SPC}{2}
\pgfmathsetmacro{\MC}{0}

%gold-speaker-1 label:95
\node[inner sep=0pt] at (15.8,\SPA+3){\includegraphics[width=13cm,height=1.4cm]{figures/95.png}};
\node[align=left] at (-3.0,\SPA) (0) {\textbf{Speaker 1:}};
\node[inner sep=0pt] at (0.1,\SPA) (G1) {};
\node[inner sep=0pt] at (1.5,\SPA) (G2) {};
\node[inner sep=0pt] at (9.8,\SPA) (G3) {};
\node[inner sep=0pt] at (11.3,\SPA) (G4) {};
\node[inner sep=0pt] at (16.5,\SPA) (G5) {};
\node[inner sep=0pt] at (22.2,\SPA) (G6) {};
\node[inner sep=0pt] at (27.7,\SPA) (G7) {};
\node[inner sep=0pt] at (30.0,\SPA) (sc) {\textbf{F-score}};

\draw[<->, >=stealth] (G1) -- node [midway,above,align=center] {devo} (G2);
\draw[<->, >=stealth] (G2) -- node [midway,above,align=center] {comprare} (G3);
\draw[<->, >=stealth] (G3) -- node [midway,above,align=center] {il} (G4);
\draw[<->, >=stealth] (G4) -- node [midway,above,align=center] {pane} (G5);
\draw[<->, >=stealth] (G5) -- node [midway,above,align=center] {ogni} (G6);
\draw[<->, >=stealth] (G6) -- node [midway,above,align=center] {giorno} (G7);

%model
\node[align=left] at (-3.0,\MA) (0) {\textbf{Model:}};
\node[inner sep=0pt] at (0.0,\MA) (a1) {};
\node[inner sep=0pt] at (4.2,\MA) (a2) {};
\node[inner sep=0pt] at (4.2,\MA) (b1) {};
\node[inner sep=0pt] at (12.6,\MA) (b2) {};
\node[inner sep=0pt] at (10.8,\MA+.5) (c1) {};
\node[inner sep=0pt] at (13.2,\MA+.5) (c2) {};
\node[inner sep=0pt] at (15.0,\MA) (d1) {};
\node[inner sep=0pt] at (19.2,\MA) (d2) {};
\node[inner sep=0pt] at (20.4,\MA+.5) (e1) {};
\node[inner sep=0pt] at (24.6,\MA+.5) (e2) {};
\node[inner sep=0pt] at (23.4,\MA) (f1) {};
%\node[inner sep=0pt] at (27.7,\MA) (f2) {};
\node[inner sep=0pt] at (28.4,\MA) (f2) {};
\node[inner sep=0pt] at (30.0,\MA) (sc1) {54.3};

\draw[<->, >=stealth] (a1) -- node [midway,above,align=center] {devo} (a2);
\draw[<->, >=stealth] (b1) -- node [midway,above,align=center] {comprare} (b2);
\draw[<->, >=stealth] (c1) -- node [midway,above,align=center] {il} (c2);
\draw[<->, >=stealth] (d1) -- node [midway,above,align=center] {pane} (d2);
\draw[<->, >=stealth] (e1) -- node [midway,above,align=center] {ogni} (e2);
\draw[<->, >=stealth] (f1) -- node [midway,above,align=center] {giorno} (f2);

\draw (-4.5,\MA-1) -- (31,\MA-1);

%gold-speaker-2 label:93
\node[inner sep=0pt] at (10,\SPB+3){\includegraphics[width=8.5cm,height=1.4cm]{figures/93.png}};

\node[align=left] at (-3.0,\SPB) (0) {\textbf{Speaker 2:}};
\node[inner sep=0pt] at (3.0,\SPB) (G12) {};
\node[inner sep=0pt] at (3.8,\SPB) (G22) {};
\node[inner sep=0pt] at (9.2,\SPB) (G32) {};
\node[inner sep=0pt] at (11.6,\SPB) (G42) {};
\node[inner sep=0pt] at (15.1,\SPB) (G52) {};
\node[inner sep=0pt] at (17.1,\SPB) (G62) {};
\node[inner sep=0pt] at (19.8,\SPB) (G72) {};
\node[inner sep=0pt] at (30.0,\SPB) (sc22) {\textbf{F-score}};

\draw[<->, >=stealth] (G12) -- node [midway,above,align=center] {devo} (G22);
\draw[<->, >=stealth] (G22) -- node [midway,above,align=center] {comprare} (G32);
\draw[<->, >=stealth] (G32) -- node [midway,above,align=center] {il} (G42);
\draw[<->, >=stealth] (G42) -- node [midway,above,align=center] {pane} (G52);
\draw[<->, >=stealth] (G52) -- node [midway,above,align=center] {ogni} (G62);
\draw[<->, >=stealth] (G62) -- node [midway,above,align=center] {giorno} (G72);

%model
\node[align=left] at (-3.0,\MB) (0) {\textbf{Model:}};
\node[inner sep=0pt] at (3.3,\MB+.5) (a12) {};
\node[inner sep=0pt] at (4.0,\MB+.5) (a22) {};
\node[inner sep=0pt] at (2.2,\MB) (b12) {};
\node[inner sep=0pt] at (8.4,\MB) (b22) {};
\node[inner sep=0pt] at (6.6,\MB+.5) (c12) {};
\node[inner sep=0pt] at (9.0,\MB+.5) (c22) {};
\node[inner sep=0pt] at (10.0,\MB) (d12) {};
\node[inner sep=0pt] at (13.2,\MB) (d22) {};
\node[inner sep=0pt] at (13.2,\MB) (e12) {};
\node[inner sep=0pt] at (16.5,\MB) (e22) {};
\node[inner sep=0pt] at (16.5,\MB) (f12) {};
%\node[inner sep=0pt] at (19.8,\MB) (f22) {};
\node[inner sep=0pt] at (19.9,\MB) (f22) {};
\node[inner sep=0pt] at (30.0,\MB) (sc12) {62.1};

\draw[<->, >=stealth] (a12) -- node [midway,above,align=center] {devo} (a22);
\draw[<->, >=stealth] (b12) -- node [midway,above,align=center] {comprare} (b22);
\draw[<->, >=stealth] (c12) -- node [midway,above,align=center] {il} (c22);
\draw[<->, >=stealth] (d12) -- node [midway,above,align=center] {pane} (d22);
\draw[<->, >=stealth] (e12) -- node [midway,above,align=center] {ogni} (e22);
\draw[<->, >=stealth] (f12) -- node [midway,above,align=center] {giorno} (f22);

\draw (-4.5,\MB-1) -- (31,\MB-1);

%gold-speaker-1 label:92
\node[inner sep=0pt] at (13.7,\SPC+3){\includegraphics[width=11.2cm,height=1.4cm]{figures/92.png}};

\node[align=left] at (-3.0,\SPC) (0) {\textbf{Speaker 3:}};
\node[inner sep=0pt] at (0.0,\SPC) (G13) {};
\node[inner sep=0pt] at (0.5,\SPC) (G23) {};
\node[inner sep=0pt] at (7.4,\SPC) (G33) {};
\node[inner sep=0pt] at (7.9,\SPC) (G43) {};
\node[inner sep=0pt] at (11.4,\SPC) (G53) {};
\node[inner sep=0pt] at (16.0,\SPC) (G63) {};
\node[inner sep=0pt] at (19.0,\SPC) (G73) {};
\node[inner sep=0pt] at (23.5,\SPC) (G83) {};
\node[inner sep=0pt] at (30.0,\SPC) (sc3) {\textbf{F-score}};

\draw[<->, >=stealth] (G13) -- node [midway,above,align=center] {devo} (G23);
\draw[<->, >=stealth] (G23) -- node [midway,above,align=center] {comprare} (G33);
\draw[<->, >=stealth] (G33) -- node [midway,above,align=center] {il} (G43);
\draw[<->, >=stealth] (G43) -- node [midway,above,align=center] {pane} (G53);
\draw[<->, >=stealth] (G53) -- node [midway,above,align=center] {ogni} (G63);
\draw[<->, >=stealth] (G63) -- node [midway,above,align=center] {ogni} (G73);
\draw[<->, >=stealth] (G73) -- node [midway,above,align=center] {giorno} (G83);

%model
\node[align=left] at (-3.0,\MC) (0) {\textbf{Model:}};
\node[inner sep=0pt] at (0.0,\MC) (a13) {};
\node[inner sep=0pt] at (2.7,\MC) (a23) {};
\node[inner sep=0pt] at (2.7,\MC) (b13) {};
\node[inner sep=0pt] at (8.1,\MC) (b23) {};
\node[inner sep=0pt] at (6.8,\MC+.5) (c13) {};
\node[inner sep=0pt] at (8.1,\MC+.5) (c23) {};
\node[inner sep=0pt] at (10.2,\MC) (d13) {};
\node[inner sep=0pt] at (12.9,\MC) (d23) {};
\node[inner sep=0pt] at (13.8,\MC) (e13) {};
\node[inner sep=0pt] at (17.0,\MC) (e23) {};
\node[inner sep=0pt] at (17.0,\MC+0.5) (f13) {};
\node[inner sep=0pt] at (20.4,\MC+0.5) (f23) {};
\node[inner sep=0pt] at (18.9,\MC) (g13) {};
%\node[inner sep=0pt] at (23.5,\MC) (g23) {};
\node[inner sep=0pt] at (23.9,\MC) (g23) {};
\node[inner sep=0pt] at (30.0,\MC) (sc13) {70.9};

\draw[<->, >=stealth] (a13) -- node [midway,above,align=center] {devo} (a23);
\draw[<->, >=stealth] (b13) -- node [midway,above,align=center] {comprare} (b23);
\draw[<->, >=stealth] (c13) -- node [midway,above,align=center] {il} (c23);
\draw[<->, >=stealth] (d13) -- node [midway,above,align=center] {pane} (d23);
\draw[<->, >=stealth] (e13) -- node [midway,above,align=center] {ogni} (e23);
\draw[<->, >=stealth] (f13) -- node [midway,above,align=center] {ogni} (f23);
\draw[<->, >=stealth] (g13) -- node [midway,above,align=center] {giorno} (g23);



\end{tikzpicture}

==> removed.tex <==
\iffalse
\begin{algorithm}[b]
\caption{Hard-EM.}\label{alg:emcur}
\begin{algorithmic}
\Procedure{Hard-EM}{$n, \mathcal{D}, t$}
%\State{$m \gets \max \lbrace{\vert e_d \vert}: e_d \in \mathcal{D} \rbrace$}
\LineComment{Init}
\For{$d \in \mathcal{D}$}
\State{$\mathbf{x}_d, \mathbf{y}_d
%, \mathbf{k}_d 
\gets \text{argmax} \delta(x,y,i,\vert s_d \vert, \vert e_d \vert)$}
\EndFor

%\State{$\mathcal{D}_c \gets \lbrace d \in \mathcal{D}: \vert e_d \vert \leq c \rbrace$} %\Comment{Select data samples.}
\For{$j \in [1,t]$} %\Comment{EM iterations}
\LineComment{M-step}
\State{$\mathcal{K} \gets \lbrace k_i \mid \exists e, \mathbf{s}, x,y \in \mathcal{D}:  p(e \vert k_i)p(k_i \vert s_x \ldots s_y) > 1 \rbrace$}
%%\LineComment{Collect prototype examples.}
\For{$k \in \mathcal{K}$}
\State{$s^k \gets \dba(s^{k_i}, \forall i : k_i \in k)$}
%%\Comment{Get prototype by summing examples.}
\EndFor
\LineComment{E-step}
\For{$d \in \mathcal{D}$}
%%\State{Find argmax alignment  based on examples.}
\State{$\mathbf{x}_d, \mathbf{y}_d, \mathbf{k}_d \gets \text{argmax} \prod_{i=1}^{\vert e_d \vert} p(e_i \vert k)p(k \vert \mathbf{s}_d)$}
\EndFor
\EndFor
%\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}
\fi 
\iffalse
\subsection{IBM Models 1 and 2 combined with HMMs}

Again, we have 
\[
\mathcal{L}(\theta \vert \mathcal{D}) = \prod_{n=1}^N\prod_{i=1}^{\vert e_n \vert } 
t(e_i \vert k_{e_i})p(k_{e_i}\vert s_{x_i} \ldots s_{y_i})
\]
\[
%\times q(x_i,y_i \vert i,\vert k_{e_i} \vert , \vert e_n \vert)
\times \delta(x_i,y_i \mid  i,\vert s_n \vert , \vert e_n \vert)
\]

But now this $k_{e_i}$ is realised with an HMM with Gaussian emmissions.
\fi

\iffalse
\section{Model: From English words to Spanish Speech}
\[
\mathcal{L}(\theta \vert \mathcal{D}) = \prod_{n=1}^Np(\mathbf{s}\vert \mathbf{e})
\]

For each English word $e_i \in \mathbf{e}$ we assume a pronunciation $b_i \in \mathcal{B}$. The whole signal must have been generated by concatenating the pronunciations of the words, however, we have to take into account the possible reordering


\[
\mathcal{L}(\theta \vert \mathcal{D}) = \prod_{n=1}^N\prod_{i =1}^{\vert e_n \vert}p(\mathbf{s}\vert b_i)p(b_i \vert e_i)
\]


\[
\mathcal{L}(\theta \vert \mathcal{D}) = \prod_{n=1}^N\sum_{B \in \mathcal{B}}p(\mathbf{s}\vert B)p(B \vert \mathbf{e})
\]
\fi

\iffalse
\subsection{Curriculum learning}

Curriculum learning \cite{bengio2009curriculum} is the method of processing the training examples in a meaningful order, trying to imitate the way that humans are taught, eg. in schools. Such a ``meaningful order" usually means in ascending order of difficulty, and in our case an intuitive measure of the difficulty of aligning a training sample would be the length of its translation.

\hl{TO-DO: Other applications of curriculum learning. (vision)}

Consider a Spanish utterance and its translation. If the length of the translation is only one word, then it is intuitive to assume that the whole speech segment is a Spanish word or phrase. Having learned good alignments for ``simple" examples, it should be easier to align ``harder" training samples.
%Therefore, that speech segment is a suitable candidate for a spanish prototype that is translated to this english word.
%\footnote{This assumes clear data: problems arise when we have imperfect transcriptions/translations or short pauses in the middle of the utterance.}

We can include curriculum learning within the standard EM algorithm by selecting the data to take into account in each iteration. A simple strategy would be to increment the amount of data that we take into account every $c$ iterations. Therefore, if in iteration $l$ we have only used data whose translation length is up to $k$, in iteration $l+c$ we will also include the training samples with translation length $k+1$.
\fi 

==> tables/griko-table.tex <==
\begin{tabular}{{@{}l|lll@{}}}
\toprule
Method & Precision & Recall & F-score \\ 
\midrule
our model & \textbf{56.6} & 51.2 & \textbf{53.8} \\
\midrule
Naive Baseline & 42.2 & \textbf{52.2} & 46.7 \\
%Naive Baseline & 37.9 & 46.8 & 41.9 \\
Attentional Model & 24.6 & 30.0 & 27.0 \\
\bottomrule
\end{tabular}
\caption{On the Griko-speech-to-Italian alignment task in the extremely low-resource setting, our model outperforms the neural attentional model and the naive baseline.}
\label{tab:griko-results}


==> tables/results-table.tex <==
\begin{center}
\begin{tabular}{{@{}ll|lll@{}}}
\toprule
 & method & precision & recall & F-score \\ 
\midrule
\multirow{3}*{\rotatebox{90}{\parbox{1.5cm}{\centering spa-eng (CALLHOME 2k)}}} &  ours & \textbf{38.8} & 38.9 & \textbf{38.8} \\
%\cmidrule{2-5}
%Naive Baseline & 17.5 & 19.2 & 18.3 \\
&naive & 31.9 & \textbf{40.8} & 35.8\\
%Naive Baseline & 26.0 & 34.7 & 29.7\\
&neural & 23.8 & 29.8 & 26.4 \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\parbox{1.4cm}{\centering spa-eng (CALLHOME all)}}}  & ours & \textbf{38.4} & 38.8 & \textbf{38.6} \\
%\cmidrule{2-5}
%Naive Baseline & 17.5 & 19.2 & 18.3 \\
&naive  & 31.8 & \textbf{40.7} & 35.7\\
%Naive Baseline & 28.1 & 35.8 & 31.4\\
&neural & 26.1 & 32.9 & 29.1 \\

\midrule
\multirow{3}{*}{\rotatebox{90}{\parbox{1.4cm}{\centering spa-eng (Fisher)}}}  & ours & \textbf{33.3} & 28.7 & \textbf{30.8} \\
&naive  & 24.0 & \textbf{33.2} & 27.8\\
& & & &\\

\midrule 
\multirow{3}{*}{\rotatebox[origin=c]{90}{gri-ita}} &
ours & \textbf{56.6} & 51.2 & \textbf{53.8} \\
%\cmidrule{2-5}
&naive & 42.2 & \textbf{52.2} & 46.7 \\
%Naive Baseline & 37.9 & 46.8 & 41.9 \\
&neural & 24.6 & 30.0 & 27.0 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Our model achieves higher precision and F-score than both the naive baseline and the neural model on all datasets.}
\label{tab:results}


==> tables/spa-2000-table.tex <==
\begin{tabular}{{@{}l|lll@{}}}
\toprule
Method & Precision & Recall & F-score \\ 
\midrule
our model & \textbf{38.8} & 38.9 & \textbf{38.8} \\
\midrule
%Naive Baseline & 17.5 & 19.2 & 18.3 \\
Naive Baseline & 31.9 & \textbf{40.8} & 35.8\\
%Naive Baseline & 26.0 & 34.7 & 29.7\\
Attentional Model & 23.8 & 29.8 & 26.4 \\
\bottomrule
\end{tabular}
\caption{In the Spanish-speech-to-English alignment task on the sample 2000 sentences, our model performs better than both the naive baseline and the neural attentional model by 3\% and 12.4\%.}
\label{tab:spanish-2000-results}


==> tables/spa-all-table.tex <==
\begin{tabular}{{@{}l|lll@{}}}
\toprule
Method & Precision & Recall & F-score \\ 
\midrule
our model & \textbf{38.4} & 38.8 & \textbf{38.6} \\
\midrule
%Naive Baseline & 17.5 & 19.2 & 18.3 \\
Naive Baseline & 31.8 & \textbf{40.7} & 35.7\\
%Naive Baseline & 28.1 & 35.8 & 31.4\\
Attentional Model & 26.1 & 32.9 & 29.1 \\
\bottomrule
\end{tabular}
\caption{In the Spanish-speech-to-English alignment task on all 17532 sentences, our model performs better than both the naive baseline and the neural attentional model by 2.9\% and 9.5\%.}
\label{tab:spanish-all-results}


==> tikzpic/scatter-small.tex <==
1 4.3 a
2 5.1 a
3 5.7 a
4 6.3 a
5 6.8 a
6 7.1 a
7 7.2 a
8 7.2 a
9 7.2 a
10 7.2 a
11 7.5 a
12 7.8 a

==> tikzpic/word-level-hist.tex <==
\begin{tikzpicture}
\begin{axis}[
    %symbolic x coords={0,5,10,15,20,25,30,35,40,45,50,55,60,65,70,75,80,85,90,95,100,105,110},
    bar width=5,
    %ticks=none,
    ytick style={draw=none},
    xtick style={draw=none},
    xlabel = {word length},
    ylabel = {Average F-score}]
    
    %xtick=data]
    \addplot[ybar,fill=white] coordinates {
    ( 2.5 , 0.4772727325 )
( 12.5 , 0.348784524584 )
( 17.5 , 0.310874467486 )
( 22.5 , 0.360605132141 )
( 27.5 , 0.407423487974 )
( 32.5 , 0.467496962534 )
( 37.5 , 0.379088031522 )
( 42.5 , 0.444365356156 )
( 47.5 , 0.571251777952 )
( 52.5 , 0.560101739534 )
( 57.5 , 0.627362117339 )
( 62.5 , 0.660948281382 )
( 67.5 , 0.630226199756 )
( 72.5 , 0.720078877559 )
( 77.5 , 0.644372116031 )
( 82.5 , 0.450878003338 )
( 87.5 , 0.735009895336 )
( 92.5 , 0.456617272179 )
( 97.5 , 0.660259161006 )
( 102.5 , 0.552785207539 )
( 112.5 , 0.833952599758 )
    };
\end{axis}
\end{tikzpicture}

==> tikzpic/word-level-scatter.tex <==
\begin{tikzpicture}
\begin{axis}[%
    scatter/classes={%
    a={mark=o,draw=black},
    b={mark=*,draw=black}},
    ylabel={F-score},
    xlabel={average word length}]
\addplot[scatter,only marks,%
    scatter src=explicit symbolic]%
table[meta=label] {
x y label
3 0.4772727325 b
10 0.394275129258 b
11 0.312990648588 b
14 0.339087795905 a
15 0.302844939794 b
16 0.331571182632 a
17 0.237937756468 a
18 0.392227692618 a
19 0.28979076592 b
20 0.178782442797 a
21 0.252216803191 a
22 0.387733074924 a
23 0.538340625527 a
24 0.445952714264 a
25 0.342013108123 a
26 0.368258182133 a
27 0.442407948741 a
28 0.480602968602 b
29 0.403835232269 a
30 0.313704499444 a
31 0.530407865855 a
32 0.701127874608 a
33 0.528348955879 b
34 0.263895616885 a
35 0.0434112105243 b
36 0.293107278328 a
37 0.5438308947 a
38 0.604097965627 a
39 0.410992808433 a
40 0.434732687641 a
41 0.275938799077 a
42 0.575790929239 a
43 0.449991950155 a
44 0.48537241467 a
45 0.758589975206 b
46 0.371454530084 a
47 0.540695537126 a
48 0.541425698119 a
49 0.644093149227 a
50 0.387605600149 a
51 0.763124141336 a
52 0.593992749021 a
53 0.612857469418 a
54 0.442928737748 a
55 0.675301981455 a
56 0.520395943163 a
57 0.580996580896 a
58 0.616582618901 a
59 0.74353346228 a
60 0.706053994444 a
61 0.706167770052 a
62 0.805749104204 a
63 0.447235045401 a
64 0.639535492808 a
65 0.451651881426 a
66 0.7553358211 a
67 0.564169766331 a
68 0.655513125018 a
69 0.724460404904 a
70 0.74010154915 a
71 0.637181130558 b
72 0.839252338056 b
73 0.566938536435 a
74 0.816920833597 a
75 0.798635664406 a
76 0.587208619263 a
77 0.592483246657 a
78 0.497277450872 a
79 0.746255598959 a
80 0.655888845231 a
81 0.520363738526 a
82 0.71937394416 a
83 0.209234942218 a
84 0.149528546556 a
85 0.777192984684 b
87 0.667556766107 b
88 0.910232384706 b
89 0.585057445849 a
90 0.76571680714 b
92 0.488192971572 b
93 0.115942037826 b
96 0.660259161006 b
100 0.185654016582 b
101 0.445424290124 b
102 0.834788147223 b
103 0.745274376225 b
110 0.833952599758 b

%\input{scatter-small.tex}
};
\end{axis}
\end{tikzpicture}

==> tikzpic/word-level-uniq.tex <==
\begin{tikzpicture}
\begin{axis}[%
    scatter/classes={%
    c={mark=o,draw=black}},
    %b={mark=*,draw=black}},
    ylabel={F-score},
    xlabel={word length}]
\addplot[scatter,only marks,%
    scatter src=explicit symbolic]%
table[meta=label] {
x y label
128 0.680412371134 c
44 0.686567164179 c
46 0.583333333333 c
72 0.628571428571 c
46 0.718446601942 c
52 0.804347826087 c
77 0.973333333333 c
70 0.0 c
52 0.831460674157 c
43 0.788732394366 c
51 0.0 c
18 0.578947368421 c
55 0.8 c
44 0.857142857143 c
79 0.835978835979 c
82 0.987654320988 c
72 0.8 c
19 0.210526315789 c
51 0.0 c
93 0.512 c
73 0.491017964072 c
57 0.609625668449 c
65 0.771653543307 c
56 0.981818181818 c
11 0.379310344828 c
59 0.757894736842 c
71 0.797752808989 c
86 0.735294117647 c
122 0.680412371134 c
71 0.818181818182 c
56 0.4 c
22 0.628571428571 c
77 0.987179487179 c
59 0.866666666667 c
39 0.583333333333 c
55 0.696202531646 c
55 0.736842105263 c
48 0.0 c
47 0.0 c
67 0.372093023256 c
33 0.825 c
60 0.811881188119 c
52 0.96 c
46 0.105263157895 c
51 0.205128205128 c
51 0.871794871795 c
61 0.300751879699 c
31 0.826666666667 c
80 0.87323943662 c
44 0.318181818182 c
89 0.988636363636 c
36 0.727272727273 c
60 1.0 c
59 0.917431192661 c
73 0.832 c
44 0.826923076923 c
46 0.708333333333 c
95 0.863636363636 c
53 0.905982905983 c
85 0.87417218543 c
53 0.39603960396 c
56 0.0 c
49 0.74358974359 c
69 0.913907284768 c
51 0.948453608247 c
106 0.0 c
14 0.0 c
43 0.68253968254 c
38 0.541353383459 c
51 0.708860759494 c
81 0.608695652174 c
49 0.697247706422 c
51 0.583333333333 c
34 0.666666666667 c
30 0.0 c
41 0.418181818182 c
82 0.959064327485 c
47 0.930693069307 c
64 0.962406015038 c
3 0.0 c
87 0.3961352657 c
42 0.894736842105 c
15 0.555555555556 c
58 0.504347826087 c
66 0.95652173913 c
97 0.74025974026 c
83 0.543859649123 c
21 0.0 c
33 0.58407079646 c
37 0.450704225352 c
42 0.743362831858 c
89 0.844720496894 c
58 0.8 c
136 0.692307692308 c
73 0.622641509434 c
49 0.515151515152 c
56 0.728971962617 c
52 0.168674698795 c
61 0.929824561404 c
48 0.842105263158 c
30 0.571428571429 c
74 0.806451612903 c
78 0.96 c
79 0.946107784431 c
87 0.994219653179 c
56 0.388888888889 c
76 0.0 c
21 0.25 c
27 0.6 c
78 0.760975609756 c
43 0.924731182796 c
70 0.947368421053 c
27 0.0 c
35 0.813953488372 c
47 0.989247311828 c
58 0.966666666667 c
69 0.0 c
58 0.896551724138 c
45 0.8 c
13 0.393939393939 c
36 0.738095238095 c
51 0.653846153846 c
52 0.0 c
78 0.78125 c
45 0.989010989011 c
101 0.696774193548 c
34 0.9375 c
58 0.974789915966 c
38 0.76 c
98 0.905027932961 c
69 0.83950617284 c
115 0.973214285714 c
67 0.695652173913 c
110 1.0 c
28 0.0 c
62 0.487804878049 c
34 0.0 c
82 0.788461538462 c
81 0.875 c
79 0.871428571429 c
31 0.246575342466 c
71 0.0 c
33 0.255319148936 c
25 0.581395348837 c
76 0.762430939227 c
37 0.232558139535 c
110 0.960698689956 c
75 0.880597014925 c
99 0.377049180328 c
50 0.412698412698 c
72 0.368794326241 c
109 0.83422459893 c
76 0.642857142857 c
56 0.788461538462 c
79 0.770731707317 c
50 0.900900900901 c
90 0.837209302326 c
27 0.486486486486 c
41 0.493150684932 c
73 0.780748663102 c
%\input{scatter-small.tex}
};
\end{axis}
\end{tikzpicture}
